GraCIAS: Grassmannian of Corrupted Images for Adversarial Security

Input transformation based defense strategies fall short in defending against strong adversarial attacks. Some successful defenses adopt approaches that either increase the randomness within the applied transformations, or make the defense computationally intensive, making it substantially more challenging for the attacker. However, it limits the applicability of such defenses as a pre-processing step, similar to computationally heavy approaches that use retraining and network modifications to achieve robustness to perturbations. In this work, we propose a defense strategy that applies random image corruptions to the input image alone, constructs a self-correlation based subspace followed by a projection operation to suppress the adversarial perturbation. Due to its simplicity, the proposed defense is computationally efficient as compared to the state-of-the-art, and yet can withstand huge perturbations. Further, we develop proximity relationships between the projection operator of a clean image and of its adversarially perturbed version, via bounds relating geodesic distance on the Grassmannian to matrix Frobenius norms. We empirically show that our strategy is complementary to other weak defenses like JPEG compression and can be seamlessly integrated with them to create a stronger defense. We present extensive experiments on the ImageNet dataset across four different models namely InceptionV3, ResNet50, VGG16 and MobileNet models with perturbation magnitude set to {\epsilon} = 16. Unlike state-of-the-art approaches, even without any retraining, the proposed strategy achieves an absolute improvement of ~ 4.5% in defense accuracy on ImageNet.

==> Sections/Background.tex <==
This section describes the problem setup and then briefly introduces the attacks used to evaluate our defense, \emph{mix to match}.

\subsection{Problem Setup}
Given a trained deep network, an adversary can add an imperceptible perturbation to the input sample that forces the model to make a wrong prediction. For a given sample $\bx$, an adversary generates a sample $\hat{\bx}= \bx+ \delta$ such that its label $l(\cdot)$ does not match that of the original sample, i.e., $l(\bx) \neq l(\hat{\bx})$. Thus the objective of an attacker can be understood as follows
\begin{align}
    \arg \max \calL(\bx+\delta,y) \;\; &  s.t. \norm{\delta}_p< \epsilon
\end{align}
Here, $y=l(\bx)$ is the ground truth label of sample $\bx$, $\delta$ is the added perturbation and $\epsilon$ is the perturbation bound.

%  Given a trained deep neural network on multi-class image classification task,  
%  we aim to evaluate the robustness of the network at inference time in presence of an adversary.  Given a test sample from the dataset of class $l(\bx)$, an adversary can generate a sample $\hat{\bx}$ such that $l(\bx) \neq l(\hat{\bx}$ while $||\bx-\hat{\bx}||_2 \leq \epsilon$. 
% Given a trained deep network for multi class image classification task. 
The aim of this work is to develop an input transformation that can pre-process an image before feeding it to the network for classification with the goal of rendering the attack ineffective. 

\subsection{Attack Methods}
While there is a huge pool of adversarial attacks that have been proposed in the literature, we briefly discuss the ones that are used in this work.

\noindent\textbf{FGSM
\cite{Fellow2014explaining}} is a one step attack method that uses gradient sign information to perturb an image with $\epsilon$ and is given by $\hat{\bx} = x+\epsilon*sign(\nabla(\calL(x,y)))$.


\noindent \textbf{PGD \cite{madry2018towards}} is an iterative attack method to generate the perturbation followed by projecting it on the constraint neighbourhood. The perturbed image is given by $\hat{\bx}^{t+1} = Proj(x^{t}+\epsilon_{step}*\nabla(\calL(x,y))$. Here, $\epsilon_{step}$ is smaller than $\epsilon$ and $Proj$ projects the sample in the norm bound and valid pixel range.

\subsection{Attacker's Knowledge}
The existing adversarial attacks can be categorized as black box and white box depending on adversaries knowledge. 

\noindent \textbf{Black Box Setting.} In this setting, the adversary does not have access to the network architecture or the parameters of the target model. In such cases, the attackers rely on a substitute network to design adversarial perturbations for the target model.

\noindent \textbf{White Box Setting.} This is stronger than the black box setting where the adversary has access to model architecture, parameters as well as training data.

\subsection{Adaptive Attacks} 
In the most general setting, in addition to the model and training data, the adversary has access to the defense strategy. If the defense operation is differentiable, the adversary can backpropagate through it along with the network, and can therefore generate a stronger attack to break the defense. 
% In order to create a stronger attack, the adversary can also have access to the defense strategy. The attacker essentially considers the transformation as part of the network and provided the operation is differentiable, can back propagate to get the gradient information to generate strong attack. 
More recently, \cite{athalye2018obfuscated} proposed two adaptive attacks allowing to approximate the gradient in case of random or non-differentiable transformation. The first approach is Backward Pass Differentiable Approximation (BPDA), which approximates the gradient for backward pass for a non-differentiable transform. Given a non-differentiable transformation $f(x)$, one can learn a network that approximates a transform, however, using identity function $x= f(x)$ during backprop is sufficient to generate strong attacks, while using transformed image as input. Another approach is Expectation Over Transformation (EOT) that essentially accounts for randomness in the transformation by using the average gradient over multiple run of transforms to approximate the gradient for attack. 


==> Sections/PreviousWork_v1.tex <==




The vulnerability of neural networks to adversarial perturbations has led the growth of a large number of defense strategies. Given the large volume of work in this area, we categorize the literature into two broad groups and briefly review recent developments in them. 

%Existing work in defense techniques can be listed under three categories. 
\noindent\textbf{Robust Training and Network Modification.} Robust training refers to strategies that retrain a model with an augmented training set. The most popular strategies use adversarial training \cite{madry2018towards,goodfellow2014explaining,kurakin2017adversarial}, where adversarially perturbed samples are included in the training set on the fly, i.e., during the model training. This approach, while effective, is very computationally expensive, as the attacks have to be regenerated multiple times during the entire training process. There exist approaches that modify the model architecture to defend against adversarial perturbations. For example \cite{xie2019feature} added feature denoising blocks in the model to circumvent the impact of noisy feature maps as a consequence of adversarial perturbations at the input. Both these sets of approaches assume access to the model and the training data. This may be too strong a constraint for deployed models, especially with an increasing number of deep learning systems being adopted for different applications. An alternate defense strategy could be one that is extrinsic to the model, e.g., an add-on pre-processing block. 

\noindent\textbf{Input Transformations.} The limitations in the previous category are addressed by input transformation based approaches, that focus on denoising the image before feeding it to the network for classification. Most defenses in this category, like the ones proposed in \cite{guo2018countering}, e.g., image compression, bit depth reduction, image quilting etc., lead to \emph{obfuscated gradient}, a way of gradient masking that gives a false sense of security. Such defenses have limited robustness on a given model under powerful attacks \cite{athalye2018obfuscated}. Other approaches that have been successful to some extent under strong attacks, for example Barrage of Random Transforms (BaRT) \cite{BOT2019} follow a highly randomized approach to choose at random from an \emph{enormous} pool of transformations, making it difficult for the attacker to break this defense. BaRT requires the model to be finetuned on the input transformations to reduce the drop in performance on clean samples. On the other hand, \cite{jpeg_dnn_cvpr19} improves the standard JPEG compression to tackle the adversarial attack while retaining the performance of clean samples to large extent. Other approaches that devise successful defense assume access to the training set. They either learn valid range spaces of clean samples or use the training set to approximate the image manifold, on which the input image is projected  \cite{samangouei2018defensegan,song2018pixeldefend}.  

Our proposed approach \textit{Mix to Match} is also an input transformation based approach. However, as opposed to existing approaches, the defense strategy is not only agnostic to model but also training data as well. 
% Another line of works focus more explicitly to project the adversarial sample on clean data image manifold. Since, the  data manifold is not known, approaches like \cite{dubey2019defense} aim to approximate the manifold
% Several approaches have been proposed in this category that aim to project the adversarial image on to the data manifold. More recently, the work in \cite{dubey2019defense} approximate the manifold projection by searching in the large database, that are used instead of adversarial image for classification.

% \textcolor{red}{While adversarial training has shown to be effective against the strongest of the attack. However all these attacks are limited to gradient perturbation  and often only robust to few perturbations, For example, adversarial trained model on high frequency data performs poorly on low frequency corrputed images. Several other  limitations of adversarial training can be listed. }

% Several other works, involve Gaussian or randomized noise to achieve robustness to adversarial perturbations.  Approaches like \cite{weng2018evaluating,ford2019adversarial} use Gaussian data augmentation over adversarial training for improved robustness of the model. In the similar way, effect of randomized smoothing has been studied by several works.

==> Sections/additional.tex <==
\section{Applications}
% GraCIAS has achieved state-of-the-art results across different models on ImageNet dataset across different attacker strength. With this success, we also see the potential of it being used as a data augmentation technique in network training. Additionally, it can also be used as an image processing tool prior to processing with simpler defense to boost their performance. 
\begin{wraptable}{r}{0.6\textwidth}
     \centering
     \begin{tabular}{c|ccc}
     \hline
        Datasets & ImageNet & ImageNet & CIFAR10\\
         Model & InceptionV3 & ResNet50 & ResNet \\\hline
         Original & 78 & 76&94.6 \\
          With Defense &62.8 &53.4 & 55.5\\\hline 
     \end{tabular}
     \caption{Classification Accuracy on Clean Samples with \textbf{GraCIAS} defense. The drop is expected on clean samples as the network has not seen such transformation during network training}
     \label{tab:clean}
 \end{wraptable}{}
\begin{figure}{r}[h]
    \centering
    \includegraphics[width= 0.45\textwidth]{plots/cifar_fgsm_m2m.png}
    % \includegraphics[width= 0.45\textwidth]{plots/cifer_bpda_eps.png}
    \caption{CIFAR10 Dataset: Performance of JPEG vs JPEG+GraCIAS as defense for different values of  $\epsilon$. The merit of combining with GraCIAS is more evident for larger adversarial perturbation.}
    % (Right) Defense Accuracy under BPDA for varying magnitude of $\epsilon$. Std. Model is the original model and  'GraCIAS trained' is the model trained with GraCIAS transformation as data augmentation for training. }
    \label{fig:cifar_bpda}
\end{figure}

% \begin{wraptable}{r}{0.6\textwidth}
%      \centering
%      \begin{tabular}{c|ccc}
%      \hline
%         Datasets & ImageNet & ImageNet & CIFAR10\\
%          Model & InceptionV3 & ResNet50 & ResNet \\\hline
%          Original & 78 & 76&94.6 \\
%           With Defense &62.8 &53.4 & 55.5\\\hline 
%      \end{tabular}
%      \caption{Classification Accuracy on Clean Samples with \textbf{GraCIAS} defense. The drop is expected on clean samples as the network has not seen such transformation during network training}
%      \label{tab:clean}
%  \end{wraptable}{}
%  \vspace{-0.4cm}

==> Sections/algo.tex <==
\begin{algorithm}[h!]
	{\small
		\caption{$\our$ Defense}
			\textbf{Input:} Adversarial sample $\bx_p$,\\
			$ e_{range}$:, range to choose for energy value to define the subspace\\ $k_{range}$: range to choose for seting the number of corrupted images \\
			\textbf{Output:} Transformed sample $\hat{\bx_p}$ for feeding to neural network for classification
		\begin{enumerate}
	\item Obtain $k$ images from $\bx_p$ by convolving with the set of $k$ random kernels as given in \ref{eq:ptrb_images}. Here $k\in k_{range}$
    \item Vectorize each image and stack to form the data matrix $X \in \bbR^{k \times 3mn}$, where $k$ is the number of images.
    \item Center and standardize the data and compute the covariance matrix. % Compute the average image and standard deviation to center the data and standardize and obtain the correlation matrix.
    \item Compute the principal components by eigendecomposition of the covariance matrix. % Compute the Eigenvalues and Eigenvectors of the correlation matrix and sort by decreasing eigenvalue.
    \item Select the first $d$ principal components that captures energy $e$, sampled uniformly from $e_{range}$. % Select first $d$ Eigenvectors to form the basis of subspace that captures maximum $e \in e_{range}$ variance in the data.
    \item Project the vectorized sample $x_p$ to obtain the low dimensional mapping $\hat{x}= U^\top x_p$, where $U$ is the basis the subspace. 
    \item Reconstruct the sample as $\hat{x}_p = U U ^\top \hat{x}$
\end{enumerate}
		}
\end{algorithm}

==> Sections/redundant.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\textwidth]{plots/Defense_overview(2).png}
    \caption{An overview of proposed Mix to Match (M2M) defense strategy is shown for an adversarial sample. The number of filters K used for creating the corrupted image image set is selected at random from a fixed range. These image are used to estimate a d dimensional subspace that is used for obtaining the low dimensional representation followed by inverse transform to obtain a rectified image. }
    \label{fig:app}
\end{figure*}

Adversarial attacks are small imperceptible perturbations carefully crafted to modify an image that can mislead the classification ability of state of the art deep neural networks. Robustness of deep learning models to such attacks \cite{Fellow2014explaining,moosavi2016deepfool,carlini2017adversarial,Fellow2013} is an active research field owing to the extensive deployment of deep learning based systems in real world applications to either automate tasks or to augment human abilities. Since these applications range from autonomous driving \cite{xu2017end} to medical evaluations \cite{bar2015deep}, the robustness of these models to adversarial perturbations is a crucial aspect for their reliability.


Consequently, recent years have witnessed the growth of several adversaries \cite{moosavi2016deepfool,Fellow2014explaining} to explore the robustness of deep models as well as defense strategies to mitigate their effect. Most prominently, the efficacy of a trained model is evaluated under white box attacks, where the adversary has access to model parameters, training data as well as the defense strategy. Similarly, several defense strategies have been developed that can broadly be grouped into two categories. Approaches in the first category have focused on making the model robust by incorporating adversarial training, modifying the network architecture itself or the loss function, followed by re-training or fine-tuning of the model. The most effective strategy in this category has been adversarial training \cite{kurakin2017adversarial,madry2018towards} that uses adversarial samples along with the clean samples to impart robustness to the network. While these approaches are effective and achieve state of the art results on small datasets like CIFAR10 and MNIST datasets, their scalability to larger datasets like ImageNet is challenging due to huge computational resources and time requirement. 

% Apart from the extensive resource requirements of these approaches, another severe limitation of their applicability in systems that have already been deployed. Therefore, there has been significant interest in the second category of approaches, where a pre-processing step is applied to the input data before feeding them to a network.
On the other hand, the second category comprises of approaches that work as pre-processing step to treat the adversarial samples with a transformation before feeding them to the network. Importantly, such approaches are best suited for real world applications, as they are agnostic to  model architecture and attack methods and therefore can be readily integrated with systems already deployed. The existing literature comprises of several input transformation based defense strategies \cite{guo2018countering,dziugaite2016study, liu2019feature,prakash2018deflecting} to remove the adversarial perturbation from the input data. However, more recently it was shown that most of these existing transforms lead to obfuscated gradient and can be overcome by stronger adversaries. Another set of approaches in this category are driven by the hypothesis that adversarial perturbations moves the image away from the data manifold. The defense strategy is designed either with an aim to approximate a cleaner sample by reconstructing from the projection in range space of clean samples  \cite{samangouei2018defensegan} or by approximating it with samples from the training image database itself \cite{dubey2019defense}. However, given the ongoing rapid advancements, dependence of defense on training data can also be exploited to develop strong adversaries. 

In this work, we propose a novel and simple input transformation \textit{Mix to Match} that depends solely on the input adversarial sample to develop, thus  making it completely agnostic to model as well as training data. The proposed defense uses a low dimensional subspace representation to reconstruct the input image mitigating the effect of adversarial noise. The subspace is approximated by corrupted versions  of an input adversarial sample and is shown to lie within close proximity of a subspace created from corrupted images of the corresponding clean sample, thereby validating the choice of our input transforms. Additionally, the proposed defense also benefits from the success of randomness in defense strategies explored earlier \cite{xie2018mitigating,BOT2019}, and is randomly parametrized both in terms of subspace dimension as well as number of image corruptions. We show that the proposed transform can withstand different magnitude and strength of attacks. 

The overall contribution of the work can be summarized as follows
\begin{itemize}
    \item The proposed defense achieves state of the art results on ImageNet dataset for both ResNet50 and IncpetionV3 models with $~ 4.5 \%$ improvement in the overpowered attack scenario.
    \item As opposed to state of the art randomized input transformation approaches, \emph{Mix to Match} benefits from not only from its intrinsic random parametrization, but also from the theoretical evidence that ensures suppression of adversarial noise. 
    \item Due to its simplicity and computational efficiency, the proposed defense can be integrated with existing weak defenses like JPEG compression to create stronger defenses, as shown in our experiments.
\end{itemize}{}
% Mixing the adversarial sample noise with random image corruptions to define a subspace to obtain the low dimensional representation.T
% he low dimensional subspace estimated from an a adversarial sample is shown to lie closer to clean sample subspace that computed by mixing the adversarial noise with randomized image corruptions  and is shown to 
% inThe proposed approach drives it strength from  image perturbed with adversarial noise, a subspace is estimated from the set of perturbed images obtained by mixing adversarial noise with random image corruptions to obtain the low dimensional representation. 

% with agnostic to to mixes adversarial noise with image corruptions to characterize a low dimensional subspace that is shown to be closer to subspace obtained from clean sample to find a lo w diemnsional prjction obtain a denoised sample by reconstructing from the low dimensional projection.



% In this work, motivated by the manifold hypothesis, we propose a novel and simple image transformation, \textit{Mix to Match} that mixes a given sample with several filtered versions to characterize a subspace for projection that is close in terms of manifold distance to the subspace of clean sample.  The proposed transformation uses a random dimensionality parameter for subspace approximation as well as a random set of filtered images to leverage the strength of randomness in transformations, which has been shown to substantially improve the robustness of deep networks \cite{xie2018mitigating,BOT2019}.
% % compute a mapping that matches the clean sample. that can be to approximate a re-projection subspace to mitigate the perturbation introduced by the attacker.

% Therefore, owing to the simplicity of the proposed transformation, which makes our defense strategy agnostic to both, model as well as the training data, we show that it can be effectively used with any deployed model. Secondly, we also show that similar to adversarial training, the proposed transformation can be used as data augmentation to train a robust network, given enough resources.
% , the same transformation can also be used as data augmentation to finetune a network.
% Lastly, owing to its only sample dependence, the performance of this defense is stable with transferable attacks.  The proposed approach provides an effective solution to adversarial attacks, while also considering the obfuscated gradient that can result in failed defense. Additionally, we show that the distance between the subspaces obtained with filtering operation on a clean and the corresponding adversarial sample are in close proximity, promising the projection of adversarial sample close to clean sample.

% This work roposes a novel input transformation based defense strategy that utilizes auto-correlation of a sample, to eliminate the noise introduced by attacker. We observed that owing to its sample dependence, the defense strategy is fairly stable across different perturbations and also model agnostic.


% Our contributions are summarized below
% \begin{itemize}
%     \item We proposed an adaptive randomized sample dependent input transformation that can account for obfuscated gradients in white box attack as well as strong adversary that is aware of defense strategy
%     \item Our proposed defense is complementary to other defense strategies, hence can be combined to make a strong defense
%     \item We show that the proposed defense is extendable to huge image datasets like ImageNet.
%     \item The proposed defense is agnostic to both the target model as well as attacker.
% \end{itemize}

%  end several input transformation based approaches \cite{guo2018countering, } have been proposed that work as a pre-processing step to clean the image before feeding the sample to the network.
%  For example the random crops can be defeated by considering expectation over transformations to compute the gradient for the attacker. Therefore highly randomized approaches like \cite{}
% Deep learning models are vulnerbable to small perturbation in image that that are imperceptible to humans but fool the model to misclassify the image. adversarial attacks alter the image with small imperceptible perturbations that can fool the model to misclassify the given image.

% Most importantly,  the robustness of these vision based system in real world applications that range from autonomous driving \cite{} to medical evaluations \cite{}, is a crucial aspect for their reliability. Therefore, 
% Due to this, recent years have studied strong adversaries that have access to trained classifier and training data as well as defense
% growth of various attack approaches to evaluated the models robustness as well various defense strategies to cope up with these attacks. Existing defense strategies can be grouped in two categories. The first set of approaches, require model or training strategy modifications to empower the model against attacks. Among these approaches, adversarial training has been the state of the art for a long time. However, recently its limitation due to overfitting has 
% perturbations that can be generated without model information, referred to as black box attacks or that can leverage the model parameters, referred as white box attack.
% threat models to evaluate the efficacy of models as well as defense strategies to counter these attacks. ...

% thier robu Due to vulnerability of model performance due to small changes in pixels, is limiting the deployment of these models, increasing the gap between human and machine perception.

% Most of the existing input transformation based strategy lead to obfuscated gradient to claim adversarial robustness, but have been circumvented with a stronger attack in white box setting as pointed by . Owing to this, any successful defense strategy should overcome white box attacks where the attacker has access to model, trained parameters and the defense strategy. Therefore, given a defense strategy an attacker that can perform the necessary approximation to devise stronger attack. For example, the randomness in the input transformation can be attacked with expectation over transforms and non-differentiable defenses with approximated gradient.  Thereafter, to overcome such adversaries, \cite{} proposed to combine a huge pool of input transformations statistically, that also accounted for obfuscated gradients and reported improved performance under high perturbation magnitudes. 



% Driven by the hypothesis that adversarial perturbations moves the data away from the manifold, approaches like \cite{} utilize the neighborhood of a given sample from the database to estimate the projection.  While it has been shown to work well, the dependence on large web database poses a challenge in integrating in existing framework.
% Our approach is also inspired by the manifold hypothesis, but uses the sample 
% Several manifold based defense approaches have been proposed that focus on putting the data back onto the manifold, More recently, work in \cite{} utilizes the neighbour sin the database to estimate the projection. While it has shown to work well, the dependence on large web database poses a challenge in 
% The proposed approach is shown to perform against the strong attacks. 
% More importantly, adversarial training was considered as state of the art approach for defense, but is recently shown to be lacking in several aspects, opening the aveneues to develop new approaches. It was shown recently shown by \cite{}, that adversarial training is not a true representative of generalization and could be defenseless for some attack. Secondly, adversarial training is computationally intesive for high dimensional images as well as large datasets, by increasing the fine-tuning time by many folds. 


% The intuition is that by selecting a random number of filters to create the set of filtered images to compute a subspace of random dimension q for low dimensional projection followed by image restoration filters out the adversarial noise in the high frequency components that are left out.
% PCA is a linear dimensionality reduction technique that can used to find a low dimensional subspace that captures the critical information in the data with maximum variance. However, using the naive PCA based image restoration is an invertible process, making it a weak defense strategy. Therefore, there are two important questions that need to be answered for effective design of the defense strategy. Firstly, how is the set of datapoints chosen that is critical to define the low dimensional subspace. And Secondly, how to make the defense strategy harder to be broken by a strong adversary.

% Therefore, relying on training data is a deterministic choice. To combat this we propose to utilize different corrupted versions of a given sample to obtain the datapoints for subspace approximation. Given an adversarially perturbed image, a set of images are generated by convolving it with random kernels of fixed size. Creating the set of images  this way, not only addresses the issue of deterministic set of images but also adds randomness in the process, which is a key component in designing a success defense strategy. Further the dimensionality of the subspace is also chosen at random depending on the given sample. The details of the same are discussed below.

% \subsubsection{Mix to Match Channel Randomness (M2M3)}
% We extend the M2M defense to M2M3 to make an effective defense against strong adaptive attacker. This requires a small modification, such that the three channels of a given sample are convolved with different random filters as oppose to use of same random filter across the channels in case of M2M defense.  




% Representing, an image of $m \times n \times 3$ as $3mn$-dimensional vector, we stack these images together and apply PCA to generate orthogonal subspace of dimension $d$. The dimension $d$ is chosen at random based on given sample to preserve a energy value sampled from a plausible range. The range is selected such that the orthogonal subspace captures the variance in the data while neglecting the high frequency components that correspond to noise. The adversarial image is first projected onto this subspace to obtain the low dimensional representation followed by inverse PCA to reconstruct the image, thus reducing the effect of noise.

==> tables/choice.tex <==
\begin{wraptable}{r}{0.4\textwidth}
    \centering
     \caption{Ablation Study of  parameter selection on defense accuracy under BPDA attack with $\epsilon=16$ for 300 images of ImageNet dataset on InceptionV3 model}
    \begin{tabular}{|ccc|}
    \hline
        Subspace & No. of & Defense\\
        Dimension& Filters&Accuracy  \\\hline
        Fixed  & Fixed &  \\
        Fixed  & Random & \\
        Random & Fixed & \\
        Random & Random & \\
        \hline
    \end{tabular}
    \label{tab:check_random}
\end{wraptable}

